Can Foundation Models Wrangle Your Data?

Foundation Models (FMs) are models trained on large corpora of data that, at very large scale, can generalize to new tasks without any task-specific finetuning. As these models continue to grow in size, innovations continue to push the boundaries of what these models can do on language and image tasks. This paper aims to understand an underexplored area of FMs: classical data tasks like cleaning and integration. As a proof-of-concept, we cast five data cleaning and integration tasks as prompting tasks and evaluate the performance of FMs on these tasks. We find that large FMs generalize and achieve SoTA performance on data cleaning and integration tasks, even though they are not trained for these data tasks. We identify specific research challenges and opportunities that these models present, including challenges with private and domain specific data, and opportunities to make data management systems more accessible to non-experts. We make our code and experiments publicly available at: https://github.com/HazyResearch/fm_data_tasks.

==> figs/guidingfigure.tex <==
\begin{figure*}[t]
    \includegraphics[width=6.75in]{figs/guiding_figure.png}
    % \includegraphics[width=6.75in]{figs/banner_sketch.jpg}
    \centering
    % \vspace{-1.5em}
    \caption{
      % \dan{Sketch below for reference, status of real figure above.}
      Guiding example of cleaning and matching task
    }
    %\vspace{-1.0em}
    \label{fig:guidingfigure}
\end{figure*}

==> figs/scaling_plots.tex <==
\begin{figure*}[t!]
    \includegraphics[width=\textwidth]{figs/scaling_plots_img.pdf}
    % \includegraphics[width=6.75in]{figs/banner_sketch.jpg}
    \centering
    % \vspace{-1.5em}
    \caption{
      % \dan{Sketch below for reference, status of real figure above.}
      Scaling Plots
    }
    %\vspace{-1.0em}
    \label{fig:scaling_plots}
\end{figure*}

==> sections/approach.tex <==
%!TEX root = ../main.tex
\section{Foundation Models for Data Tasks}
\label{sec:approach}
This section will describe how we use prompting for the data cleaning and integration tasks.
% This is the nuts and bolts methods section.

\subsection{Data Tasks as Prompting Tasks}
This section explain how all tasks can be cast as generation tasks using yes/no questions. Described the basic format for each task. %Doesn't go into details for how we represent entities, points to~\cref{subsec:schema} for more details on that. 
\subsection{Prompt Construction}
Discuss (1) prompt construction principles and (2) human-in-the-loop prefix construction process. We will tie prefix / prompt principles back to rule / hand-crafted features in Section 2.1. %Doesn't go into details for how we represent entities, points to~\cref{subsec:schema} for more details on that. 
 

% \subsection{Schema-agnostic Representations}~\label{subsec:schema}
% Discuss how to represent entities with natural language representations (row serialization). Highlight difference with Ditto representations that use [COL] tokens, or rule-based method that rely on schema-specific configuration files (e.g. which field to match together for EM). 

% \subsection{Knowledge Transfer}
% % \ines{TBD what goes in here, maybe talk about internal vs external knowledge, and few-shot with prefix here?}
% Discuss prompt engineering principles and the effect of the prefix in priming the model for the given task. Tie prefix / prompt principles back to rule / hand-crafted features in Section 2.1.

==> sections/exp.tex <==
%!TEX root = ../main.tex

\input{tables/reasoning}
\input{tables/schema}
\input{tables/global_results_imp}

\input{tables/global_results}
\input{tables/prompt_ablation}


\section{Experiments}
\label{sec:exp}

\subsection{Setup}
This section describes the different datasets, model variants (2.7B, 6.7B, 20B and 175B) and evaluation metrics for each task.
\subsubsection{Models}
\subsubsection{Datasets}
\subsubsection{Metrics}


\subsection{Results}
\subsubsection{Demonstration of Unified Interface}
This section describes the main results for FMs -- they lead to SotA results with few or limited training examples~(\cref{tab:global}). We compare with previous SOTA approaches, and perform a scale (\# of parameters)  and context size (\# labelled examples) analysis.


\input{figs/scale}
\subsubsection{Demonstration of Domain Knowledge}
This section describes the main results for FMs -- they l
Show qualitative experiments highlighting reasoning and knowledge capabilities as a function of effects of scale (see Table~\cref{tab:reasoning}):
\begin{itemize}
    \item zip code to city integrity constraint (see ~\cref{tab:reasoning})
    \item schema annotation (column type detection)
    \item semantic mismatch (see ~\cref{tab:reasoning})
\end{itemize}

\subsubsection{Demonstration of Schema-transfer}
This section compare FMs to ditto (SOTA EM system), on task transfer abilities (see Table~\cref{tab:schema}).

% \subsubsection{Quantitative Results}

% This section describes the main results for FMs -- they lead to SotA results with few or limited training examples~(\cref{tab:global}). We compare with previous SOTA approaches.
% \begin{itemize}
%     \item Sota numbers on Entity Matching \item Sota numbers on Imputation /  error detection
%     \item Sota numbers on Schema Matching?
% \end{itemize}

% \subsubsection{Qualitative Results}
% Show qualitative experiments highlighting reasoning and knowledge capabilities as a function of effects of scale:
% \begin{itemize}
%     \item zip code to city integrity constraint (see ~\cref{tab:reasoning})
%     \item schema annotation (column type detection)
%     \item semantic mismatch (see ~\cref{tab:reasoning})
% \end{itemize}



% \subsection{Analyses}
% \subsubsection{Scale analysis (\#parameters)} How does scale effect qualitative and quantitative performance?:
% \begin{itemize}
%     \item Qualitative understanding: common knowledge (e.g., zipCode), entity relations (e.g., mapping from area code to city, attribute type relations)
%     \item Quantitative performance, knowledge intensive tasks, how do we do when \# parameters change
% \end{itemize}

% \subsubsection{Context Size (\# labelled examples)}
% How many examples are needed to do well with few shots, how do we pick these examples? 

% \subsubsection{Schema Agnosticism}
% Compare FMs to existing deep learning methods 

% \begin{comment}


% \subsubsection{Potential experiments list}
% \begin{itemize}
%     \item \textbf{Can FMs be used as a unifying interface for data integration tasks?}
%         \begin{itemize}
%             \item Simple interface that lets us get SOTA (prompt + prefixes)
%             \item Demonstration of encoding human / domain information with natural language
%                 \begin{itemize}
%                     \item Show how traditional data constraints (from the cleaning literature) can be cast as a natural language prompt 
%                     \item Show how dataset specific relations can be encoded 
%                 \end{itemize}
%         \end{itemize}
%   \item \textbf{What do these models know and reason about, and what are the tradeoffs with scale?}
%         \begin{itemize}
%             \item Knowledge analyses (imputation ablations): 
%                 \begin{itemize}
%                     \item Qualitative examples (model knows about common knowledge: e.g., zipCode) 
%                     \item Entity relations (e.g., mapping from area code to city, attribute type relations)
%                 \end{itemize}
%             \item Reasoning analyses (prefix ablations on entity or schema matching, and data constraint ablations for cleaning): 
%                 \begin{itemize}
%                     \item K=0 to K=5, how much does it rely on prefixes to do the matching?
%                     \item Constraint understanding (e.g, ZIP codes in a certain range)
%                     \item Functional data dependency (e.g., co-occurrences between attributes)
%                     \item Cross-dataset prefix: does it need to see the same schema in the prefix to reason about matching?
%                     \item \textit{note: for (2) and (3) we will run ablations over the dependencies and constraints in the holoclean paper}
%                 \end{itemize}
%             \item Scaling experiments (tradeoffs between accuracy and scale):
%                 \begin{itemize}
%                     \item number of paramters
%                     \item number of  datapoints (prefixes), zero/few shot
%                 \end{itemize}
%         \end{itemize}
%   \item \textbf{What are the limitations and common failure modes of this approach, and how can we fix them?}
%         \begin{itemize}
%             \item Knowledge failures:
%                 \begin{itemize}
%                     \item Public/Private Knowledge: could we build a synthetic example to show the failure mode? Maybe Simran\'s benchmark.
%                     \item Temporal data (e.g., old area codes): \textbf{Maybe train a small model where we show how we selectively update area code information?}
%                 \end{itemize}
%             \item Reasoning failures:
%                 \begin{itemize}
%                     \item Where / when does the latent model reasoning fail? Demonstrate through case examples.
%                     \item Create hard synthetic reasoning examples.
%                 \end{itemize}
%             \item Scale and cost limitations:
%                 \begin{itemize}
%                     \item Can we transfer only the knowledge we need on a smaller foundation model?
%                     \item Are there cheaper alternatives? \textbf{Adapter experiments as a cost effective alternative}.
%                 \end{itemize}
%         \end{itemize}
% \end{itemize}
% \end{comment}

% Summary of the claims we want to show:
% \begin{itemize}
%     \item Unagi encompasses many DB tasks and custom-built solutions. For example, we can do all the deep learning entity matching papers in the same framework---with minimal changes in configs between them.
%     % \item Unagi enables many DB tasks with simple configs---show all the datasets we can run, with line counts of the configs for each one
%     \item You might expect that we would sacrifice performance as a result of this simple interface, but Unagi achieves SoTA on these classic database tasks, like entity matching, data cleaning, and relation extraction.
%     \item Unagi's contrastive interface allows targeted correction of failure modes after error analysis (e.g., one entity matching task has trouble with remixes, so we add a contrastive head separating remixes from non-remixes).
%     \item Finally, training with Unagi is cheap---we achieved these SoTAs on pre-emptible GPUs for less than a cup of coffee.
% \end{itemize}

% % \dan{Prose verison of above bullets}
% % In this section, we validate that Unagi can specify models for a variety of data management tasks with minimal code.
% % Despite this simplicity, models trained with Unagi achieve state-of-the-art performance on a variety of data management tasks, including entity matching, data cleaning, and...---in one case achieving perfect performance where previous state-of-the-art had \num{5.6}\% error rate.
% % We demonstrate that Unagi's simple multitask contrastive interface allows for rapid exploration of training strategies to address specific failure modes, which is critical to achieving this performance.
% % We present case studies where Unagi enables up to \num{3.5} points of improvement in performance over defaults with less than 10 lines of Python code.

% \subsection{Applications}

% \input{tables/datasets}

% Unagi can train models for a wide variety of data management applications with minimal configuration.
% In this section, we describe three benchmark applications that we use to demonstrate the expressivity of the Unagi framework: entity matching, data cleaning, and relation extraction.
% Table~\ref{tab:datasets} lists the datasets we use for evaluation (more TBD) across three applications, as well as the size of the configs necessary to run each application.

% \subsubsection{Entity Matching}
% We use the benchmark datasets from Ditto and DeepMatcher \todo{CITE}, which contain two tasks: EM-Structured and EM-Textual.
% Each dataset contains records from two sources.
% The task is to label a pair of records as representing the same entity as not.
% We fine-tune a BERT classifier and follow the strategy from Ditto to encode records for the task: we... \todo{describe}


% \subsubsection{Data Cleaning}
% We use benchmark datasets from TabReformer.
% \todo{Add these, run them}

% \subsubsection{Relation Extraction}
% We use TACRED and Re-TACRED.
% \todo{Add these}

% % \subsection{Case Studies: Reproducing Custom-Built Solutions}
% % In this section, we describe case studies where we use Unagi to reproduce custom-built solutions for our datasets.
% % The goal of this is to give examples of a bunch of papers that had to build custom solutions, where we can encompass their whole thing in a tiny config.
% % Systems that we can replicate with small configs:
% % \begin{itemize}
% %     \item Ditto: SoTA cross-encoder for entity matching, 1-line config
% %     % \item Ember: bi-encoder for entity matching, 1-line config
% %     \item TabReformer: SoTA encoder for data cleaning, 1-line config
% %     \item RoBERTa-large-typed-marker: SoTA for relation extraction (among those that have released their code), 1-line config
% % \end{itemize}

% \subsection{Performance}

% We show that \sysname\ achieves SoTA everywhere!

% \subsubsection{Entity Matching}
% \input{tables/em_perf.tex}

% Table~\ref{tab:em_perf} shows the performance of Unagi on the entity matching data sets.
% Despite Unagi's simple interface, models trained with Unagi match or achieve state-of-the-art performance on \num{all} data sets---outperforming custom-built solutions such as Ditto and DeepMatcher, as well as general-purpose systems such as Ember.

% \subsubsection{Data Cleaning}

% \input{tables/dc_perf.tex}

% \subsubsection{Relation Extraction}

% \input{tables/re_perf.tex}

% \subsection{Case Studies: Domain Knowledge}

% Case studies in how we incorporate domain knowledge with the tabular interface.

% \input{tables/targeted_perf}

% A key feature of the Unagi framework is the ability to examine model errors and correct them using the contrastive interface.
% Table~\ref{tab:targeted_perf} shows case studies where we use Unagi's contrastive interface to correct failure modes, as well as the number of lines of Python code necessary to achieve the lift.
% In the remainder of this section, we discuss \num{2} concrete examples and show pseudocode for the examples; in the first, we use the multitask framework 

% \subsubsection{iTunes-Amazon}

% \input{tables/itunes_amazon_errors}
% \input{listings/itunes_amazon}

% The iTunes-Amazon dataset seeks to match songs between an iTunes catalogue and an Amazon Music catalogue.
% Table~\ref{tab:itunes_amazon_errors} shows three errors from a model trained with the default Unagi config.
% A common failure mode is when one of the songs is a remix (for example, ``We Dem Boyz (Louis Futon Remix)'' is not the same song as ``We Dem Boy'').
% To address this failure mode, we wrote a simple function to identify when the word ``remix'' appeared in either song in a candidate entity match pair.
% We used this feature, along with the original label, to supervise an additional contrastive head.
% The pseudocode to detect this new feature is shown in Listing~\ref{lst:itunes_amazon}.
% % Figure~\num{XX} shows the result of this intervention in the embedding space; the model learns to treat match pairs with the string ``remix'' differently from those without.
% As a result, the model can distinguish between remixes and non-remixes of the same song during entity matching, resulting in \num{3.5} points of lift---a \num{66}\% error reduction.

% \subsection{Cost: Fine-tuning vs. Adaptors}

% Show tradeoffs between fine-tuning and adapting.

% \subsection{Autotuner}

% Show performance of the autotuner and the ``default'' choices.

==> sections/shaping.tex <==
%!TEX root = ../main.tex

\section{Input Shaping}
\label{sec:shaping}

In this section we discuss how we can address the challenges through input shaping.

==> tables/adapting.tex <==
%!TEX root = ../main.tex

\begin{table}[b]
    \centering
    \begin{tabularx}{\linewidth}{l|X|X|X|X}
        \Xhline{1.3pt}
        Dataset        & DITTO (all data) & GPT3-6B \ \ (0-shot) & Adaptor-6B (all data) & Adaptor-6B (100 ex)\\
         \hline
         Fodors-Zagats  & & & & \\
         Beer           & & & & \\
         iTunes-Amazon  & & & & \\
         DBLP-ACM       & & & & \\
         Walmart-Amazon & & & & \\
         DBLP-Google    & & & & \\
         Amazon-Google  & & & & \\
         \Xhline{1.3pt}
    \end{tabularx}
\caption{Adaptor performance for a stacked 6B \gpt model with a single adaptor layer in between as we decrease the amount of labeled data. We measure performance of a single adaptor trained on a single task for that task.} 
\label{tab:adaptor}
\end{table}

==> tables/global_results_errd.tex <==
%!TEX root = ../main.tex

% \begin{table}[t]
%     \centering
%     \begin{tabular}{ |c||c|c|c|  }
%     %  \hline
%     %  \multicolumn{4}{|c|}{SoTA Zero-Shot Manual Prefix (K=2)} \\
%      \hline
%      Dataset&HoloClean &HoloDeect &GPT3-175B (K=2)\\
%      \hline
%      Hospital&  94.4  & 51.4  & 97.4\\
%      \hline
%     \end{tabular}
% \caption{Results of baselines and \gpt for error detection} 
% \label{tab:global_errd}
% \end{table}

==> tables/prompt_ablation.tex <==
%!TEX root = ../main.tex

\begin{table*}[t]
    \centering
    \begin{tabular}{|l|l|ccc|ccc|ccc|}
        \Xhline{1.3pt}
        Task & Dataset  & \multicolumn{3}{c}{$k=0$} & \multicolumn{3}{c}{$k=10$, Random} & \multicolumn{3}{c}{$k=10$, Selected} \\ 
        & & 355M & 6B & 175B & 355M & 6B & 175B & 355M & 6B & 175B \\ 
        \Xhline{1.3pt}
        & Fodors-Zagats & X & X & X & 18.8 \num{$\pm$} & 57.89 \num{$\pm$} & 93 \num{$\pm$} & 20.8 & 63.15 & 100 \\ \cline{2-11}
        & Beer & X & X & X & 13.33 \num{$\pm$} & 58.53 \num{$\pm$} & 82.75 \num{$\pm$} & 36.36 & 59.25 & 96.55 \\ \hline
     \end{tabular}
\caption{Results (F1-score) of baselines and \gpt across the three tasks of entity matching, data imputation, and error detection.} 
\label{tab:prompt_ablation}
\end{table*}




==> tables/reasoning.tex <==
%!TEX root = ../main.tex

\begin{table}[b]
    \centering
    \begin{tabularx}{\linewidth}{l|X|X|XXX}
        \Xhline{1.3pt}
        Dataset & Rule Based~\cite{konda2016magellan} & Ditto~\cite{li2020deep} & \multicolumn{3}{c}{\gpt (Manual $k=2$)} \\
        & & & Sm & Md & Lg \\ \Xhline{1.3pt}
        External & & & & & \\ \hline
        Fuzzy & & & & &\\ \hline
        Exact & & & & &\\ \Xhline{1.3pt}
    \end{tabularx}
\caption{Demonstration of the reasoning capabilities of \gpt on data imputation. We measure performance on subpopulations of data that capture the \yell{X} reasoning patterns explained in \yell{X}.} 
\label{tab:reasoning}
\end{table}

==> tables/schema.tex <==
%!TEX root = ../main.tex

\begin{table}[b]
    \centering
    \begin{tabularx}{\linewidth}{l|X|X|X}
        \Xhline{1.3pt}
        Dataset & Rule Based~\cite{konda2016magellan} & Ditto~\cite{li2020deep} & \gpt (Manual $k=2$) \\ \Xhline{1.3pt}
        A $\rightarrow$ A (Strc) & & & \\ \hline
        A $\rightarrow$ B (Strc) & NA & & \\ \hline
        A $\rightarrow$ C (Text) & NA & & \\ \Xhline{1.3pt}
    \end{tabularx}
\caption{Demonstration of impact of schema / domain shift across a rule based system, a fine-tuned FM, and \gpt on entity matching. We show performance of training a model on structured entity matching dataset \yell{X} and evaluating the model on three different datasets. As \gpt requires no training, we measure its few-shot performance with manually selecting $k=2$ examples.} 
\label{tab:schema}
\end{table}

